MBIAS: Mitigating Bias in Large Language Models While Retaining Context

The deployment of Large Language Models (LLMs) in diverse applications necessitates an assurance of safety without compromising the contextual integrity of the generated content. Traditional approaches, including safety-specific fine-tuning or adversarial testing, often yield safe outputs at the expense of contextual meaning. This can result in a diminished capacity to handle nuanced aspects of bias and toxicity, such as underrepresentation or negative portrayals across various demographics. To address these challenges, we introduce MBIAS, an LLM framework carefully instruction fine-tuned on a custom dataset designed specifically for safety interventions. MBIAS is designed to significantly reduce biases and toxic elements in LLM outputs while preserving the main information. This work also details our further use of LLMs: as annotator under human supervision and as evaluator of generated content. Empirical analysis reveals that MBIAS achieves a reduction in bias and toxicity by over 30\% in standard evaluations, and by more than 90\% in diverse demographic tests, highlighting the robustness of our approach. We make the dataset and the fine-tuned model available to the research community for further investigation and ensure reproducibility. The code for this project can be accessed here https://github.com/shainarazavi/MBIAS/tree/main. Warning: This paper contains examples that may be offensive or upsetting.

==> checklist.tex <==
\section*{ACL 2024 Responsible NLP Checklist}

\textbf{A. For every submission:}
\begin{itemize}[label=\Checkedbox]
    \item \textbf{A1.} Did you describe the limitations of your work? \\
\textit{Yes, we have included a Limitations section just before the References section.  }

    \item [\Checkedbox] \textbf{A2.} Did you discuss any potential risks of your work? \\
\textit{There exists a risk that our dataset and model results could be exploited for malicious purposes, enabling groups with the intent to discreetly transmit biased messages. It is crucial to manage how users interpret these results, emphasizing that the model's output should not be accepted without critical evaluation to avoid reinforcing existing stereotypes.}
    
\item  [\Checkedbox] \textbf{A3.} Do the abstract and introduction summarize the paper’s main claims?  \\
\textit{Yes. We have included the claims in abstract and introduction. Sections 3 and 4 exhibit the evidence to our claims.}
\end{itemize}

\textbf{B. Did you use or create scientific artifacts?}
\begin{itemize}[label=\Checkedbox]
    \item \textbf{B1.} Did you cite the creators of artifacts you used?\\
\textit{Yes, we have cited the base models creators.}
    \item \textbf{B2.} Did you discuss the license or terms for use and / or distribution of any artifacts?\\
\textit{Yes, in Section 4.}
    \item \textbf{B3.} Did you discuss if your use of existing artifact(s) was consistent with their intended use, provided that it was specified? For the artifacts you create, do you specify intended use and whether that is compatible with the original access conditions?\\
\textit{Yes, where it applies, we have mentiond.}
    \item \textbf{B4.} Did you discuss the steps taken to check whether the data that was collected / used contains any information that names or uniquely identifies individual people or offensive content, and the steps taken to protect / anonymize it?\\
\textit{Yes, we implemented measures to anonymize identifiers and names within the collected data to ensure privacy. The paper's objective is to identify marginalized demographics and assess any stereotypes or potential harm directed towards them through linguistic analysis, with a focus on safeguarding their identities and maintaining confidentiality throughout. }
    \item [\Checkedbox]\textbf{B5.} Did you provide documentation of the artifacts, e.g., coverage of domains, languages, and linguistic phenomena, demographic groups represented, etc.?\\
\textit{N/A. We have, however, provided details on our artifacts in Section 3 and Appendices.}
    \item \textbf{B6.} Did you report relevant statistics like the number of examples, details of train / test / dev splits, etc. for the data that you used / created?\\
\textit{Yes, Section 5..}
\end{itemize}
\textbf{C. Did you run computational experiments?}
\begin{itemize}[label=\Checkedbox]
    \item \textbf{C1.} Did you report the number of parameters in the models used, the total computational budget, and computing infrastructure used?\\
\textit{Yes, we have mentioned these in details in Section 4.}
    \item \textbf{C2.} Did you discuss the experimental setup, including hyperparameter search and best-found hyperparameter values?\\
\textit{Yes, in Section 4.}
    \item \textbf{C3.} Did you report descriptive statistics about your results, and is it transparent whether you are reporting the max, mean, etc. or just a single run?\\
\textit{Yes, we have mentioned these related details in Section 4 and correspononding Appendices.  }
    \item \textbf{C4.} If you used existing packages, did you report the implementation, model, and parameter settings used?\\
\textit{Yes, Section 4.1.}
\end{itemize}
\textbf{D. Did you use human annotators or research with human participants?}
\begin{itemize}[label=\Checkedbox]
    \item \textbf{D1.} Did you report the full text of instructions given to participants, including any risks? \\
\textit{Yes, in Appendix B.}    \item [\Checkedbox] \textbf{D2.} Did you report information about how you recruited and paid participants, and discuss if such payment is adequate given the participants’ demographic? \\
\textit{In-house staff from different demographics volunteered to participate. More information provided in Appendix B.}
    \item [\Checkedbox] \textbf{D3.} Did you discuss whether and how consent was obtained from people whose data you’re using/curating? \\
\textit{N/A. The dataset is included as part of our larger data collection, which is licensed through legal agreements.}
    \item [\Checkedbox] \textbf{D4.} Was the data collection protocol approved (or determined exempt) by an ethics review board? \\
    \textit{N/A. The data used in this paper is our own, and part of a larger dataset, liscenced under CC BY-NC 4.0.}
    \item [\Checkedbox] \textbf{D5.} Did you report the basic demographic and geographic characteristics of the annotator population that is the source of the data? \\
\textit{N/A, they are in-house and we have mentioned their diversity.}
\end{itemize}

